Low-resource Deep Entity Resolution with Transfer and Active Learning

Entity resolution (ER) is the task of identifying different representations of the same real-world entities across databases. It is a key step for knowledge base creation and text mining. Recent adaptation of deep learning methods for ER mitigates the need for dataset-specific feature engineering by constructing distributed representations of entity records. While these methods achieve state-of-the-art performance over benchmark data, they require large amounts of labeled data, which are typically unavailable in realistic ER applications. In this paper, we develop a deep learning-based method that targets low-resource settings for ER through a novel combination of transfer learning and active learning. We design an architecture that allows us to learn a transferable model from a high-resource setting to a low-resource one. To further adapt to the target dataset, we incorporate active learning that carefully selects a few informative examples to fine-tune the transferred model. Empirical evaluation demonstrates that our method achieves comparable, if not better, performance compared to state-of-the-art learning-based methods while using an order of magnitude fewer labels.

==> macro.tex <==
%literal
\definecolor{blu}{rgb}{0.820, 0.124, 0.69} %literal
\definecolor{vio}{rgb}{0.53, 0.0, 0.69}
\definecolor{red}{rgb}{0.8, 0.0, 0.0}
%literal
\definecolor{LightGray}{gray}{0.9}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]

\newcommand{\jungo}[1]{{\color{red} [Jungo: #1]}}
\newcommand{\lucian}[1]{{\color{vio} [Lucian: #1]}}
\newcommand{\yunyao}[1]{{\color{blu} [Yunyao: #1]}}
\newcommand{\sairam}[1]{{\color{red} [Sairam: #1]}}


